EnseSmells: Deep ensemble and programming language models for automated code smells detection

A smell in software source code denotes an indication of suboptimal design and implementation decisions, potentially hindering the code understanding and, in turn, raising the likelihood of being prone to changes and faults. Identifying these code issues at an early stage in the software development process can mitigate these problems and enhance the overall quality of the software. Current research primarily focuses on the utilization of deep learning-based models to investigate the contextual information concealed within source code instructions to detect code smells, with limited attention given to the importance of structural and design-related features. This paper proposes a novel approach to code smell detection, constructing a deep learning architecture that places importance on the fusion of structural features and statistical semantics derived from pre-trained models for programming languages. We further provide a thorough analysis of how different source code embedding models affect the detection performance with respect to different code smell types. Using four widely-used code smells from well-designed datasets, our empirical study shows that incorporating design-related features significantly improves detection accuracy, outperforming state-of-the-art methods on the MLCQ dataset with with improvements ranging from 5.98% to 28.26%, depending on the type of code smell.

==> commands.tex <==
\lstset{
	basicstyle=\small\ttfamily,
	columns=flexible,
	breaklines=true,
	alsoletter={+},
}

% Minimal (M3-Rascal) syntax.
\newcommand*{\irsc}[1]{\lstinline[language=m3]+#1+} % inline manifest syntax
\lstdefinelanguage{m3}{
	basicstyle=\ttfamily\scriptsize,
	keywordstyle=\bfseries,
	keywords={m3,declarations,methodInvocation},
	literate={<-}{$\leftarrow$}{1},
	tabsize=2,
	alsoletter={-}
}

\newcommand{\code}[1]{{\small \texttt{#1}}}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\color{black} 
		\node[shape=circle,draw=cyan,fill=black!0!white,inner sep=.3pt] (char) {{{\texttt\textbf #1}}};}}
\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;} 


% Usual suspects
\usepackage{xspace}
\newcommand*{\ie}{i.e.,\@\xspace}
\newcommand*{\eg}{e.g.,\@\xspace}
\newcommand*{\cf}{cf.\@\xspace}
\makeatletter
\newcommand*{\etc}{%
	\@ifnextchar{.}%
	{etc}%
	{etc.\@\xspace}%
}
\makeatother
\newcommand*{\etal}{\emph{et~al.}\@\xspace}

\newcommand{\nb}[2]{
	\fbox{\bfseries\sffamily\scriptsize#1}
	{\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
}

\definecolor{darkgray}{gray}{0.78}
\definecolor{lightgray}{gray}{0.85}
\definecolor{verylightgray}{gray}{0.95}
\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{lightgray}{gray}{0.85}

\newcommand{\GH}{\textsc{GitHub}\xspace}
\newcommand{\GC}{\textsc{GitCNN}\xspace}
%\newcommand{\mC}{\textsc{$\mu$CNN}\xspace}
% \newcommand{\mC}{\textsc{memoCNN}\xspace}
\newcommand{\ES}{\textsc{EnseSmells}\xspace}
\newcommand{\DS}{\textsc{DeepSmells}\xspace}
\newcommand*{\AU}{AURORA\@\xspace}
\newcommand*{\TF}{TensorFlow\@\xspace}
\newcommand*{\KR}{Keras\@\xspace}

\newcommand*{\MN}{MixNet\@\xspace}
\newcommand*{\EN}{EfficientNet\@\xspace}

\newcommand*{\etclst}{\colorbox{blue!10}{\textbf{\vphantom{a}\dots}}}

\newcommand\PN[1]{\textcolor{blue}{\nb{Phuong}{#1}}}
\newcommand\LI[1]{\textcolor{gray}{\nb{Ludovico}{#1}}}
%\newcommand\CDS[1]{\textcolor{blue}{\nb{Claudio}{#1}}}


%\newcommand{\rqfirst}{\textbf{RQ$_1$}: \emph{How does \ES compare with %exhibit improvement in comparison to previous work on 
%\DS?}}


\newcommand{\rqfirst}{\textbf{RQ$_1$}: \emph{How do software metrics impact the performance enhancement of \ES?}}
\newcommand{\rqsecond}{\textbf{RQ$_2$}: \emph{How do various embedding techniques impact each category of code smell?}}
\newcommand{\rqthird}{\textbf{RQ$_3$}: \emph{How eﬀective is \ES compared with classical ML classifiers when utilizing only structural features?}}
\newcommand{\rqfourth}{\textbf{RQ$_4$}: \emph{How does \ES perform compared to the baselines?}} 


% \newcommand{\rqfirst}{\emph{RQ$_1$: How effective is \mC at classifying the considered categories?}~} %Does a deeper network help obtain a better classification performance metamodels 
% \newcommand{\rqsecond}{\emph{RQ$_2$: Which network configuration contributes to a better performance?}~} %Does a wider and deeper network contribute to a better performance?
% \newcommand{\rqthird}{\emph{RQ$_3$: How does \mC compare with \AU?}~} % in terms of prediction accuracy
% %\newcommand{\rqfourth}{\emph{RQ$_4$: Is matrix beneficial to the classification?}~} % the selection of invocations affect the

% %[boxrule=0.86pt,left=0.3em, right=0.3em,top=0.1em, bottom=0.08em]

\newtcolorbox{shadedbox}{
	drop shadow southeast,
	breakable,
	enhanced jigsaw,
	colback=white,
	boxrule=0.80pt,
	left=0.3em,
	right=0.3em,
	top=0.1em,
	bottom=0.05em
}


%\newcommand{\rqfourth}{\textbf{RQ$_4$}: \emph{Is the performance gain proportional to the number of training images?}~}
%\newcommand{\rqfifth}{\textbf{RQ$_5$}: \emph{What is the average execution time for recognizing a fruit using \EN or \MN on an ordinary computer?}~}
%\newcommand{\rqsixth}{\textbf{RQ$_6$}: \emph{Is transfer learning beneficial to the classification of fruits?}~}

